Constable: Improving Performance and Power Efficiency by Safely Eliminating Load Instruction Execution

Load instructions often limit instruction-level parallelism (ILP) in modern processors due to data and resource dependences they cause. Prior techniques like Load Value Prediction (LVP) and Memory Renaming (MRN) mitigate load data dependence by predicting the data value of a load instruction. However, they fail to mitigate load resource dependence as the predicted load instruction gets executed nonetheless. Our goal in this work is to improve ILP by mitigating both load data dependence and resource dependence. To this end, we propose a purely-microarchitectural technique called Constable, that safely eliminates the execution of load instructions. Constable dynamically identifies load instructions that have repeatedly fetched the same data from the same load address. We call such loads likely-stable. For every likely-stable load, Constable (1) tracks modifications to its source architectural registers and memory location via lightweight hardware structures, and (2) eliminates the execution of subsequent instances of the load instruction until there is a write to its source register or a store or snoop request to its load address. Our extensive evaluation using a wide variety of 90 workloads shows that Constable improves performance by 5.1% while reducing the core dynamic power consumption by 3.4% on average over a strong baseline system that implements MRN and other dynamic instruction optimizations (e.g., move and zero elimination, constant and branch folding). In presence of 2-way simultaneous multithreading (SMT), Constable's performance improvement increases to 8.8% over the baseline system. When combined with a state-of-the-art load value predictor (EVES), Constable provides an additional 3.7% and 7.8% average performance benefit over the load value predictor alone, in the baseline system without and with 2-way SMT, respectively.

==> 99_revision_summary.tex <==
% \documentclass[journal,twocolumn,10pt]{IEEEtran}
% \usepackage[letterpaper, left=0.5in, right=0.5in, bottom=0.5in, top=0.5in]{geometry}

% \usepackage{setspace}
% \setstretch{0.9}

% \makeatletter
% \let\sv@endpart\@endpart
% \def\@endpart{\thispagestyle{empty}\sv@endpart}
% \makeatother

% \hypersetup{
%     colorlinks=false,
% }

\newgeometry{margin=0.48in}
\setstretch{0.86}

\thispagestyle{empty}
\twocolumn

We thank the reviewers for their insightful feedbacks. We have addressed most feedback in the revised draft. 
%We hope you accept online and nominate for best paper. 




\section*{Common Questions}

\noindent \textbf{CQ1: Area/power modeling of Constable's structures [C,D].}
\hyperlink{rev:cq1}{\hgolden{Revised \mbox{\cref{sec:methodology_power}} and newly-added Table~\mbox{\ref{table:area_power}}}} shows Constable's area/power estimates in absolute term. We have \hyperlink{rev:cq1_2}{\hgolden{revised \mbox{\cref{sec:eval_power}}}} by taking Constable's power into consideration.

\noindent \textbf{CQ2: Wrong path execution [C,E].}
We have \hyperlink{rev:cq2_1}{\hg{revised \mbox{\cref{sec:design_design_decisions_wrong_path}}}} to clarify. We have modeled Constable without a mechanism to restore its structures on a branch misprediction recovery. 
%This is because we observe that, on average the performance of Constable when its structures are updated only by correct path instructions is only $0.2\%$ higher than when they are updated by all instructions without a restoring mechanism on branch misprediction recovery.

\noindent \textbf{CQ3: Architecting SLD [D,E]}
\hyperlink{rev:cq3_1}{\hapricot{Newly-added \mbox{\cref{sec:design_design_decisions_sld}}}} quantitatively explains this. We have modeled SLD with a limited read/write bandwidth for our evaluation.




\section*{Reviewer A}
% \noindent \xrfill{1pt} \textbf{REVIEWER A} \xrfill{1pt} \par

\noindent \textbf{A1. Clarification of figure.} 
\hyperlink{rev:a1_1}{\ho{Revised Fig.~\mbox{\ref{fig:load_port_util}}}} shows (1) the fraction of total execution cycles where at least one load port is utilized, and (2) further categorizes the load-utilized cycles based on whether or not a global-stable load utilizes a port.

\noindent \textbf{A2. Added citation} to “Characterization of Silent Stores”.

\noindent \textbf{A3. Better terminology.}
We would replace the “stable load” as “address-data invariant (ADI) load” in the final version. 
%We deferred applying the changes in the revision to keep it consistent with the older terminology.




\section*{Reviewer B}
% \noindent \xrfill{1pt} \textbf{REVIEWER B} \xrfill{1pt} \par

\noindent \textbf{B1. Benefits in register-rich architecture.}
Increasing the number of architectural registers is likely going to reduce only the number of stack loads, while the number of non-stack loads will likely see minimal changes. We verify this intuition by compiling all C/C++ workloads from SPEC CPU 2017 suite using Clang 18.1.0-rc2~\cite{clang_18} that has added support to Intel APX ISA update, which increases the number of architectural registers from 16 to 32~\cite{intel_apx}. We ran the APX-enabled workloads using the test inputs via Intel SDE 9.33~\cite{intel_sde} and collected the load count using the “-mix” flag. On average across 14 workloads running end-to-end, we see a $13.6\%$ reduction in the stack loads whereas the overall load count only reduces by $2.4\%$. Since Constable’s performance benefit not only comes from eliminating stack loads but also non-stack loads (as shown in \hyperlink{rev:b1_1}{\htan{newly-added Fig.~\mbox{\ref{fig:perf_breakdown}}}} and \hyperlink{rev:b1_2}{\hspringgreen{Fig.~\mbox{\ref{fig:cov_breakdown}}}}), we believe that Constable will continue to provide significant performance and power benefits even in a register-rich architecture. 
%We are adding support to simulate all APX instructions in our infrastructure and will add quantitative comparison in the final version.

\noindent \textbf{B2. Is Constable mostly resolving loads in tight loop?}
As \hyperlink{rev:b2_1}{\hb{newly-added Fig.~\mbox{\ref{fig:global_stable_breakdown}}(b)}} shows, the global-stable loads targeted by Constable have a wide range of inter-occurrence distance (i.e., the number of instructions between two successive dynamic instances of the same global-stable load instruction). While, $31.9\%$ of global-stable loads have less than 50 inter-occurrence distance (e.g., coming from tight loop), the remaining loads have relatively-long inter-occurrence distance (e.g., accessing global-scope variables, calling inlined functions in a loop).

\noindent \textbf{B3. Memoization and loop-transformation techniques.}
\hyperlink{foo}{\hgrey{Newly-added sections in \mbox{\cref{sec:related_works}}}} do a qualitative comparison of Constable against memoization and loop-transformation techniques.

\noindent \textbf{B4. Deeper characterization of stable loads.}
\hyperlink{rev:b2_1}{\hb{Newly-added Fig.~\mbox{\ref{fig:global_stable_breakdown}}(a) and \mbox{\ref{fig:global_stable_breakdown}}(b)}} shows a deeper characterization of global-stable loads based on their addressing mode and inter-occurrence distance. \hyperlink{rev:b1_2}{\hspringgreen{Newly-added Fig.~\mbox{\ref{fig:cov_breakdown}}}} shows the fraction of global-stable loads that are eliminated by Constable at runtime. 
%Newly-added Fig.~\ref{fig:global_stable_breakdown}(a) and (b) shows an in-depth characterization of stable-loads based on their addressing mode and inter-occurrence distance (i.e., the number of instructions between two successive occurrences of the global-stable load from the same PC), respectively. Fig. XXX(a) shows that only $20\%$ global-stable loads on average use PC-relative addressing (likely accessing variables in global scope), whereas $42.6\%$ and $37.4\%$ use stack-relative and register-relative addressing. Fig. XXX(b) shows that global-stable loads show a wide spectrum of inter-occurrence distance.

% Constable differs from memoization techniques in two key ways. First, instruction-level memoization typically waits for the value of source registers of an instruction to be available for looking up the memoization buffer to retrieve the memoized output [Sodani and Sohi, ISCA’97]. Constable explicitly tracks the changes in the source architectural registers of a likely-stable load instruction, and immediately unlocks its dependents using the last-fetched value, if both the conditions are satisfied. Second, Constable incurs significantly lower hardware overhead (15.4 KB) as compared to prior memoization techniques, which often requires a memoization buffer as big as  (or even bigger than) the L1 data cache.

% Compiler techniques like global value numbering, common subexpression elimination, and loop-invariant code motion identify pieces of code that stay invariant across various granularity of a program (e.g., basic-block, loop body, or the global scope) and eliminate their redundant execution. All the workloads used in this work are already compiled with these optimizations. We demonstrate that Constable provides performance benefits on top of such well-optimized workloads while being a purely-microarchitectural technique.




\section*{Reviewer C}
% \noindent \xrfill{1pt} \textbf{REVIEWER C} \xrfill{1pt} \par

% We thank the reviewer for the feedback. We have answered the questions in the common question section.

\noindent \textbf{C1. Constable's risk-reward trade-off.}
While Constable's performance benefit may seem small, it provides the same performance benefit as a machine with one additional load execution width as shown in Fig.~\ref{fig:sensitivity}(a).
% (which would have incurred both power and area overhead), while \emph{decreasing} the power consumption and only a moderate increase in the area. 
Scaling load execution width results in a significant \emph{increase} in core power consumption and area overhead. However, Constable provides the same performance benefit while \emph{decreasing} power consumption with a minimal area overhead.
Thus Constable provides a better design choice for improving performance than naively scaling machine resources.

\noindent \textbf{C2. Power consumed by Constable structures.}
Please see CQ1.

\noindent \textbf{C3. Handling wrong path execution.}
Please see CQ2.




\section*{Reviewer D}

\noindent \textbf{D1. Area and power analysis.}
Please see CQ1.

\noindent \textbf{D2. xPRF design.}
As DLVP~\cite{rami_ap} shows, adding a $32$-entry xPRF with 2-read/2-write ports to the existing PRF increases the combined area and the write energy by $6\%$ and $7\%$, whereas adding two additional write ports to the existing PRF increases area and write energy by $16\%$ and $51\%$, respectively.
%To reduce the xPRF's read port requirement, we add a \emph{predicted bit} 
%Since xPRF is used only for storing predictions for likely-stable loads (which is a small fraction of the total dynamic instructions), it gets written less often than the PRF. We find that two write ports for xPRF is sufficient for realizing Constable while losing only $0.2\%$ on average than a xPRF with infinite write ports. 

\noindent \textbf{D3. Coherence protocol.}
We use MESIF protocol~\cite{mesif} (\hyperlink{rev:d2_1}{\hdandelion{revised Table~\mbox{\ref{table:sim_params}}}}). The only change we need in the protocol is when a likely-stable yet not eliminated load returns from the cache hierarchy, the CV-bit corresponding to the requesting core gets pinned (meaning, a clean-eviction from the core-private cache will not reset this bit).  
%This pinning essentially represents the core’s intention to eliminate load instruction that is accessing this cache block, and the core needs to be notified when this cacheblock is getting snooped. If the cacheblock gets clean-evicted from the core-private caches, the core can still keep on eliminating the load since pinning ensures that the first snoop request to that cacheline will be delivered to the core, at which point the core will stop eliminating any further instances of that load instruction. The CV-bit will get reset normally seeing the snoop request. 
Pinning does not require extra state information.

\noindent \textbf{D4. SLD design.}
Please see CQ3.

\noindent \textbf{D5. Table 1 clarifications.}
We have \hyperlink{rev:d5_1}{\hy{revised Table~\mbox{\ref{table:storage_overhead}}}} to clarify.

\noindent \textbf{D6. RMT update.}
When a PC gets removed from an AMT entry, the \texttt{can\_eliminate} flag of the corresponding PC gets reset in the SLD, which prevents Constable from eliminating subsequent instances of the same load instruction. Thus it is not necessary to remove a PC from RMT when it gets removed from AMT entry.

\noindent \textbf{D7. PC-list replacement.}
We implement a first-in-first-out replacement policy in the PC list in RMT and AMT entries.

\noindent \textbf{D8. Confusion with ``trace" term.}
\hyperlink{rev:d8_1}{\hp{Revised \mbox{\cref{sec:methodology_workloads}}}} clarifies that our simulator faithfully models the wrong path execution. 
%We will change the term “trace” with “checkpoint” in the final version.

\noindent \textbf{D9. Writing improvement.}
We have revised the first few sections to reduce redundancy and will further polish in the final version.




\section*{Reviewer E}

\noindent \textbf{E1. Parameter passing case.}
Constable indeed eliminates the highlighted stack-loads in Fig.~\ref{fig:stable_load_example}(c) and (d) since the \texttt{rc\_shift\_low} function gets inlined (\hyperlink{rev:e1_1}{\hyo{highlighted in \mbox{\cref{sec:headroom_workload_analysis}}}}) within the body of its caller function \texttt{rc\_encode} 
%(\texttt{liblzma/rangecoder/range\_encoder.h:149}, not shown in the picture). 
(not shown in picture).
As a result, the highlighted loads are actually accessing the stack space of the caller \texttt{rc\_encode}, which does not get modified till \texttt{rc\_encode} itself returns. Since \texttt{rc\_encode} repeatedly calls \texttt{rc\_shift\_low} in a loop with the same \texttt{out} buffer pointer and \texttt{out\_size} arguments, the dynamic instances of the highlighted static load instructions get eliminated upon gaining the stability confidence.
%(barring the first few instances to gain the stability confidence).
In general, Constable can eliminate stack loads if load happens repeatedly without any changes to the stack pointers and stores to the load address. Two such cases are (1) high reuse of the same passed parameters inside function body before calling/returning from the function, and (2) an inlined function getting repeatedly called with the same parameters. \hyperlink{rev:b1_2}{\hspringgreen{Newly-added Fig.~\mbox{\ref{fig:cov_breakdown}}}} shows that Constable eliminates $45.5\%$ of global-stable stack loads.
%In general, Constable can eliminate dynamic instances of a stack load instruction if the load happens repeatedly before the function calls another function or returns. As we show in the newly-added Fig. XXX, Constable covers XXX\% of all global-stable stack-loads in the runtime.

\noindent \textbf{E2. Elimination of spill/fill loads.}
Constable cannot cover a global-stable load originating from register spilling due to \emph{silent stores}. \hyperlink{rev:b1_2}{\hspringgreen{Newly-added \mbox{\cref{sec:evaluation_load_coverage}}}} quantifies this loss of opportunity.

\noindent \textbf{E3. Understanding covered loads.}
\hyperlink{rev:b1_2}{\hspringgreen{Newly-added \mbox{\cref{sec:evaluation_load_coverage}} and Fig.~\mbox{\ref{fig:cov_breakdown}}}} discuss Constable's runtime coverage of global-stable loads and quantify loss of opportunities into various reasons.

\noindent \textbf{E4. LB entry elimination.}
We thank the reviewer for this thoughtful suggestion. Skipping LB allocation by relying on pipeline flush may result in an incorrect execution. Consider this example: at cycle $T_0$, a load instance $LD_1$ from $PC_x$ to address $A$ gets eliminated by Constable and skips LB allocation. At a later cycle $T_1$, the AMT entry for address $A$ gets evicted due to \emph{capacity miss} in AMT. At this stage, Constable looks up SLD with the PCs present in that AMT entry and resets the \texttt{can\_eliminate} flag. This prevents any subsequent instances of $PC_x$ from getting eliminated. But at a later cycle $T_2$, a store instruction older than $LD_1$ in program order resolves its store address $A$. Since $A$ is no longer present in AMT, Constable does not trigger the pipeline flush. However, the younger load $LD_1$ remained in the pipeline with an incorrect result. This scenario is caught by our functional verification methodology mentioned in \cref{sec:methodology_func_veri}. Thus, Constable cannot skip the LB allocation.

\noindent \textbf{E5. Supporting indirect accesses to SLD.}
Please see CQ2.

\noindent \textbf{E6. Handling wrong path execution.}
Please see CQ1.



% \end{document}
